Fermionic Semi-Annihilating Dark Matter

Semi-annihilation is a generic feature of dark matter theories with symmetries larger than Z2. We investigate two examples with multi-component dark sectors comprised of an SU(2)L singlet or triplet fermion besides a scalar singlet. These are respectively the minimal fermionic semi-annihilating model, and the minimal case for a gauge-charged fermion. We study the relevant dark matter phenomenology, including the interplay of semi-annihilation and the Sommerfeld effect. We demonstrate that semi-annihilation in the singlet model can explain the gamma ray excess from the galactic center. For the triplet model we scan the parameter space, and explore how signals and constraints are modified by semi-annihilation. We find that the entire region where the model comprises all the observed dark matter is accessible to current and planned direct and indirect searches.

==> Files/XSec.tex <==
\section{Annihilation Cross Sections}\label{app:xsec}

\subsection{Singlet Fermion Model}

Cover the details of semi-annihilation free of Sommerfeld complications.

A load of cross section results.  All results give only the leading term at threshold.  Throughout, $v_{fs}$ represents the velocity of the final state particles and we define
\begin{equation}
  \mu \equiv \frac{m_\phi^2}{m_\psi^2} \,.
\end{equation}
\begin{equation}
  \sigv (\bar{\psi} \psi \to \phi \phi) = \frac{3y^4v_{fs}}{32\pi m_\psi^2} \, \biggl( 1 - \frac{8}{9} \, \mu + \frac{2}{9} \, \mu^2 \biggr) \biggl( 1 - \frac{1}{2}\,\mu \biggr)^{-4} \frac{s - 4m_\psi^2}{4m_\psi^2} \,.
\end{equation}
\begin{equation}
  \sigv (\phi \phi \to \bar{\psi} \psi) = \frac{4y^4v_{fs}}{\pi m_\phi^2} \, \frac{1}{\mu} \, \biggl(1 - \frac{1}{\mu} \biggr) \,.
\end{equation}
\begin{equation}
  \sigv (\psi \psi \to \phi h) = \frac{y^2\lambda_{h\phi}^2v_{fs}}{256\pi m_\psi^2} \, \frac{v_{EW}^2}{m_\psi^2} \, \biggl( 1 - \frac{1}{4} \, \mu \biggr) \frac{s - 4m_\psi^2}{4m_\psi^2} \,.
\end{equation}
Using $\Omega = (m_\psi - m_\phi)/(m_\psi + m_\phi)$ and $\epsilon_h = 2 m_h/(m_\psi + m_\phi)$, 
\begin{equation}
  \sigv (\psi \phi \to \bar{\psi} h) = \frac{y^2\lambda_{h\phi}^2v_{fs}v_{EW}^2}{\pi(m_\phi + m_\psi)^4} \, \frac{(1 + \Omega) ((3 + \Omega)^2 - \epsilon_h^2)}{((3+\Omega)(1-\Omega)^2 - \epsilon_h^2 (1 + \Omega))^2} \,.
\end{equation}
The last case, $\phi\phi \to SM$, is well known.

\subsection{Triplet Fermion Model}

Sommerfeld calculation.

Cross sections simply related to singlet case:
\begin{align}
  \sigv (\phi \phi \to \bar{\psi} \psi) & = 3 \sigv (\phi \phi \to \bar{\psi} \psi)_{singlet} \,, \\
  \sigv (\phi \phi \to SM) & = \sigv (\phi \phi \to SM)_{singlet} \,, \\
  \sigv (\psi \phi \to \bar{\psi} h) & = \sigv (\psi \phi \to \bar{\psi} h)_{singlet} \,, \\
  \sigv (\psi \psi \to \phi h) & = \frac{1}{3} \sigv (\psi \psi \to \phi h)_{singlet} \,, \label{eq:PhiH} \\
  \sigv (\bar{\psi} \psi \to \phi \phi) & = \frac{1}{3} \sigv (\bar{\psi} \psi \to \phi \phi)_{singlet}
\end{align}

Gauge-mediated cross sections in the unbroken phase.
\begin{align}
  \sigv (\bar{\psi}\psi \to WW) & = \frac{\pi \alpha_2^2}{m_\psi^2} \,, \label{eq:WWunbroken} \\
  \sigv (\bar{\psi}\psi \to H^\dagger H) & = \frac{\pi \alpha_2^2}{12 m_\psi^2} \,, \label{eq:HHunbroken} \\
  \sigv (\bar{\psi}\psi \to \bar{f}f) & = \frac{\pi \alpha_2^2N_c}{6 m_\psi^2} \,, \label{eq:ffunbroken} \\
  \sigv (\psi\psi \to W\phi) & = \frac{\alpha_2y^2v_{fs}}{3 m_\psi^2} \,, \label{eq:WPhiunbroken} \\
  \sigv (\psi \phi \to \bar{\psi} W) & = \frac{\alpha_2y^2v_{fs}}{3} \, \frac{m_\phi^2}{m_\psi(m_\psi + m_\phi)^3} \,.
\end{align}

For the computation of the Sommerfeld enhancement, we need to break the two-fermion initial states into spin, charge and $\set{Z}_4$ subspaces.  We define the following terms that will show up in the potentials:
\begin{align}
  A(r) & = \frac{\alpha}{r} + \frac{\alpha_2c_w^2}{r} \, e^{-m_Zr} \,, \\
  B(r) & = \frac{\alpha_2}{r} \, e^{-m_Wr} \,, \\
  C(r) & = \frac{y^2}{4\pi r} \, e^{-m_\phi r} \,.
\end{align}

$Q=2$, $\set{Z}_4 = 2$: states $\{\psi^+ \psi^+, \bar{\psi}^- \bar{\psi}^-\}$.  The cross section is necessarily zero, due to there being no final states.

$Q=2$, $\set{Z}_4 = 0$: states $\{\psi^+ \bar{\psi}^-\}$.  This annihilates to $W^+W^+$ through a pure spin-0 state.  Neglecting the final state masses,
\begin{equation}
  \Gamma = \frac{\pi\alpha_2}{m_\psi^2} \,, \quad \text{and} \quad V(r) = A(r) - C(r) \,.
\end{equation}

$Q=1$, $\set{Z}_4 = 2$: states $\{ \psi^+ \psi^0 , \bar{\psi}^- \bar{\psi}^0 \}$.  The only final state is $\phi W^+$.  This has both spin-1 and spin-0 pieces, but the spin-0 piece vanishes when $m_W\to 0$.
\begin{equation}
  \Gamma = \frac{\alpha_2y^2}{2m_\psi^2} \, 
  \begin{pmatrix}
    1 & 1 \\ 1 & 1 
  \end{pmatrix} 
  \,, \quad \text{and} \quad V(r) = -
  \begin{pmatrix}
    B(r) & C(r) \\ C(r) & B(r) 
  \end{pmatrix} \,.
\end{equation}

$Q=1$, $\set{Z}_4 = 0$: states $\{ \psi^+ \bar{\psi}^0 , \psi^0 \bar{\psi}^- \}$.  These have multiple annihilation channels: $\bar{f} f'$, $W^+ h$, $W^+\gamma$ and $W^+Z$.  The first two of these are pure spin-1, the third pure spin-0 and the last a mixture of the two.
\begin{equation}
  \Gamma^{Spin-0} = \frac{\pi\alpha_2^2}{2m_\psi^2} \, 
  \begin{pmatrix}
    1 & 1 \\ 1 & 1 
  \end{pmatrix} 
  \,, \qquad \Gamma^{Spin-1} = \biggl( \frac{N_f \pi \alpha_2^2}{4m_\psi^2} + \frac{\pi \alpha_2^2}{8m_\psi^2} \biggr) 
  \begin{pmatrix}
    1 & - 1 \\ - 1 & 1 
  \end{pmatrix} \,,
\end{equation}
where $N_f$ sums over both flavour and colour.  The potential is
\begin{equation}
  V(r) = -
  \begin{pmatrix}
    C(r) & B(r) \\ B(r) & C(r)
  \end{pmatrix} \,.
\end{equation}

$Q=0$, $\set{Z}_4 = 2$: states $\{ \psi^+ \psi^-, \psi^0 \psi^0, \bar{\psi}^0 \bar{\psi}^0, \bar{\psi}^+ \bar{\psi}^- \}$.  These states can annihilate to $\phi + \{\gamma, Z, h\}$.  Note that the neutral states can only form a spin-0 state due to Fermi statistics.  However, in the limit of massless SM particles, the spin-0 annihilation cross sections vanish.  For the spin-1 subspace,
\begin{equation}
  \Gamma = \frac{\alpha_2 y^2}{2m_\psi^2} \, 
  \begin{pmatrix}
    1 & 0 & 0 & 1 \\
    0 & 0 & 0 & 0 \\
    0 & 0 & 0 & 0 \\
    1 & 0 & 0 & 1 \\
  \end{pmatrix}
  \,, \quad \text{and} \quad V(r) = - 
  \begin{pmatrix}
    A(r) & B(r) & 0 & C(r) \\
    B(r) & 0 & C(r) & 0 \\
    0 & C(r) & 0 & B(r) \\
    C(r) & 0 & B(r) & A(r) 
  \end{pmatrix} \,.
\end{equation}

$Q=0$, $\set{Z}_4 = 0$: states $\{ \psi^+ \bar{\psi}^+, \psi^0 \bar{\psi}^0, \psi^- \bar{\psi}^- \}$.  These states can annihilate to $\bar{f}f$, $\phi\phi$, $\gamma\gamma$, $ZZ$, $Z\gamma$, $Zh$, $Z\gamma$ and $W^+W^-$.  The annihilations to two gauge bosons are spin-0, and the other processes are spin-1.
\begin{equation}
  \Gamma^{Spin-0} = \frac{\pi\alpha_2^2}{2m_\psi^2} \, 
  \begin{pmatrix}
    3 & 4 & 3 \\
    4 & 4 & 4 \\
    3 & 4 & 3
  \end{pmatrix}
  \,, \qquad \Gamma^{Spin-1} = \biggl( \frac{N_f \pi \alpha_2^2}{4m_\psi^2} + \frac{\pi \alpha_2^2}{8m_\psi^2} \biggr)
  \begin{pmatrix}
    1 & 0 & -1 \\
    0 & 0 & 0 \\
    -1 & 0 & 1
  \end{pmatrix} \,,
\end{equation}
and
\begin{equation}
  V(r) = -
  \begin{pmatrix}
    A(r) & B(r) & C(r) \\
    B(r) & C(r) & B(r) \\
    C(r) & B(r) & A(r) 
  \end{pmatrix} \,.
\end{equation}

Cross-checks: if we sum these expressions for states of definite charge over all initial states and average, we should reproduce the fully unbroken phase expressions.  This sums over the diagonal elements of the $\Gamma$ matrices (including factors of 2 that are absent here) and including the charge-conjugate initial states to those explicitly listed.  For annihilations to $\phi + SM$, note that \modeqref{eq:PhiH} is pure p-wave, so we want to reproduce \modeqref{eq:WPhiunbroken}.
\begin{equation}
  \sigv = \frac{1}{9} \, \frac{\alpha_2 y^2}{m_\psi^2} \biggl( 2 \times 2 \times \frac{1}{2} \biggr\rvert_{Q=\pm 1} + 2 \times \frac{1}{2} \biggr\rvert_{Q=0} \biggr) = \frac{\alpha_2 y^2}{3m_\psi^2} \,.
\end{equation}
For annihilations to two gauge bosons, the spin-0 piece should reproduce \modeqref{eq:WWunbroken}.
\begin{equation}
  \sigv = \frac{1}{9} \, \frac{\pi\alpha_2^2}{m_\psi^2} \biggl( 2 \times 1 \rvert_{Q=\pm 2} + 2 \times 2 \times \frac{1}{2} \biggr\rvert_{Q=\pm 1} + \frac{1}{2} \times (3 + 4 + 3) \rvert_{Q = 0} \biggr) = \frac{\pi\alpha_2^2}{m_\psi^2} \,.
\end{equation}
For annihilations of gauge boson plus Higgs, or for two gauge bosons in spin-1, the total should reproduce \modeqref{eq:HHunbroken}.
\begin{equation}
  \sigv = \frac{1}{9} \, \frac{\pi\alpha_2^2}{m_\psi^2} \biggl( 2 \times 2 \times \frac{1}{8} \biggr\rvert_{Q = \pm 1} + 2 \times \frac{1}{8} \biggr\rvert_{Q = 0} \biggr) = \frac{\pi\alpha_2^2}{12m_\psi^2} 
\end{equation}
For annihilations to $ff$,
\begin{equation}
  \sigv = \frac{1}{9} \, \frac{N_c\pi\alpha_2^2}{m_\psi^2} \biggl( 2 \times 2 \times \frac{1}{4} \biggr\rvert_{Q=\pm 1} + 2 \times \frac{1}{4} \biggr\rvert_{Q=0} \biggr) = \frac{N_c\pi\alpha_2^2}{6m_\psi^2} \,.
\end{equation}
